Selective Deep Convolutional Features for Image Retrieval

Convolutional Neural Network (CNN) is a very powerful approach to extract discriminative local descriptors for effective image search. Recent work adopts fine-tuned strategies to further improve the discriminative power of the descriptors. Taking a different approach, in this paper, we propose a novel framework to achieve competitive retrieval performance. Firstly, we propose various masking schemes, namely SIFT-mask, SUM-mask, and MAX-mask, to select a representative subset of local convolutional features and remove a large number of redundant features. We demonstrate that this can effectively address the burstiness issue and improve retrieval accuracy. Secondly, we propose to employ recent embedding and aggregating methods to further enhance feature discriminability. Extensive experiments demonstrate that our proposed framework achieves state-of-the-art retrieval accuracy.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-siggraph.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> tex/discussion.tex <==
\subsection{Discussion}
\label{sec:discussion}

==> tex/evaluation-using-tine-tuned.tex <==
\subsection{Taking advantages from tine-tuned network}
Since our proposed methods take the 3D activation tensor of a convolution layer as the input, our methods are totally compatible with fine-tuned networks \cite{finetune_hard_samples,netvlad}.  In the \textbf{Fine-tuned network} section of Table \ref{tb:state-of-art}, we evaluate our best framework - $\mathcal{M}_\text{MAX} + \phi_\Delta+\psi_\text{d}$ - with the local conv. features of fine-tuned VGG for image retrieval task from \cite{netvlad,finetune_hard_samples} as input. 

Different from the results with off-the-shelf VGG network, when using local conv. features extracted from fine-tuned network from \cite{finetune_hard_samples}, our method can achieve very competitive results with those from \cite{finetune_hard_samples} at dimensionality of 512. Our method outperforms \cite{finetune_hard_samples} in majority of benchmark datasets, including {\textit{Oxford5k}}, {\textit{Oxford105k}}, {\textit{Holidays}}, and {\textit{Paris106k}}. Furthermore, at 1024 dimensionality, our method outperforms the most competitive method \cite{netvlad,finetune_hard_samples} by more than $+2.5\%$, except {\textit{Paris6k}} dataset with $+1.0\%$ performance gain to the next best \textbf{\textit{mAP}} value. It is worth to note that the end-to-end training architecture proposed in \cite{finetune_hard_samples} still inherits the drawback of upper bounded final representation dimensionality from R-MAC \cite{R-MAC}.

In Table \ref{tb:state-of-art}, ``NetVLAD fine-tuned'' represents the results reported in \cite{netvlad} after fine-tuning for differentiating the results from NetVLAD using off-the-shelf network. ``NetVLAD $\star$'' and ``siaMAC $\dagger$'' mean that the fine-tuned VGG from NetVLAD \cite{netvlad} and siaMAC \cite{finetune_hard_samples} respectively are used to extracted local conv. features as input for our proposed framework. 


% Note that we do not use re-trained model from \cite{deep_img_retr} since (i) the authors do not release the re-trained VGG model\footnote{The authors only release the re-trained ResNet \cite{resnet} model.}, and (ii) \citet{deep_img_retr} proposed to re-train the model in \textit{supervised} manner while our work mainly focus only \textit{unsupervised} aspect. We cited the results from \cite{deep_img_retr} in Table \ref{tb:state-of-art} to emphasize that our \textit{unsupervised} method can achieve a very competitive performance even with \textit{supervised} method \cite{deep_img_retr}.


% \begin{table*}[ht]
% \caption{Comparison with the state of the art.}
% \label{tb:fine-tune}
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Dim.}} & \multicolumn{5}{c|}{\textbf{Datasets}}\\
% \cline{3-7} & & \textit{\textbf{Oxford5k}} & \textbf{\textit{Oxford105k}} & \textbf{\textit{Paris6k }}& \textbf{\textit{Paris106k}} & \textbf{\textit{Holidays}} \\
% \hline
% \hline

% % MAC fine-tuned \cite{finetune_hard_samples} & 512 & 79.7 & 73.9 &  82.4 & 74.6 & 79.5 \\
% R-MAC fine-tuned \cite{finetune_hard_samples} & 512 & 77.0 & 69.2 & 83.8 & 76.4 & 82.5 \\
% NetVLAD fine-tuned \cite{netvlad} & 1024 & 69.2 & - & 76.5 & - & 86.5 \\
% % \rowcolor{Gray}
% % Deep Image Retrieval \cite{deep_img_retr} & 512 & 83.1 & 78.6 & 87.1 & 79.7 & 89.1\\
% \hline
% R-MAC fine-tuned \cite{finetune_hard_samples} + \textbf{Our-MAX mask} & 512 & 77.7 & 72.7 & 83.2 & 76.5 & 86.3 \\
% R-MAC fine-tuned \cite{finetune_hard_samples} + \textbf{Our-MAX mask} & 1024 & 81.4 & 77.4 & 84.8 & 78.9 & 88.9 \\
% NetVLAD fine-tuned \cite{netvlad} + \textbf{Our-MAX mask} & 1024 & 75.2 & 71.7 & 84.4 & 76.9 & 91.5 \\
% \hline
% \multicolumn{7}{|c|}{\textbf{Longer dimensionality}} \\
% \hline
% NetVLAD fine-tuned \cite{netvlad} & 4096 & 71.6 & - & 79.7 & - & 87.5 \\
% NetVLAD fine-tuned \cite{netvlad} + \textbf{Our-MAX mask} & 4096 & 78.2 & 75.7 & 87.8 & 81.8 & 92.2 \\
% R-MAC fine-tuned \cite{finetune_hard_samples} + \textbf{Our-MAX mask} & 4096 & 83.8 & 80.6 & 88.3 & 83.1 & 90.1 \\

% \hline
% \end{tabular}
% \end{table*}
